eCeLLM: Generalizing Large Language Models for E-commerce from Large-scale, High-quality Instruction Data

With tremendous efforts on developing effective e-commerce models, conventional e-commerce models show limited success in generalist e-commerce modeling, and suffer from unsatisfactory performance on new users and new products - a typical out-of-domain generalization challenge. Meanwhile, large language models (LLMs) demonstrate outstanding performance in generalist modeling and out-of-domain generalizability in many fields. Toward fully unleashing their power for e-commerce, in this paper, we construct ECInstruct, the first open-sourced, large-scale, and high-quality benchmark instruction dataset for e-commerce. Leveraging ECInstruct, we develop eCeLLM, a series of e-commerce LLMs, by instruction-tuning general-purpose LLMs. Our comprehensive experiments and evaluation demonstrate that eCeLLM models substantially outperform baseline models, including the most advanced GPT-4, and the state-of-the-art task-specific models in in-domain evaluation. Moreover, eCeLLM exhibits excellent generalizability to out-of-domain settings, including unseen products and unseen instructions, highlighting its superiority as a generalist e-commerce model. Both the ECInstruct dataset and the eCeLLM models show great potential in empowering versatile and effective LLMs for e-commerce. ECInstruct and eCeLLM models are publicly accessible through https://ninglab.github.io/eCeLLM.

==> intro.tex <==
With the development of the internet and digital economy, 
\mbox{e-commerce} has become ubiquitous in everyday life, 
and has been attracting increasing attention from the research community.
%
Recently, as large language models (LLMs) 
such as GPT-4~\cite{GPT4}, Claude 2~\cite{Claude2}. Gemini~\cite{team2023gemini} and LLaMA~\cite{touvron2023llama} have demonstrated exceptional performance in natural language processing (NLP)~\cite{zhao2023survey}, information retrival~\cite{spatharioti2023comparing}, among many other fields~\cite{frieder2023large,zeng2023large},   
%
significant efforts have been dedicated to adapting LLMs for \mbox{e-commerce} tasks such as recommendation~\cite{wu2023survey}.
%
Existing efforts have primarily focused on studying the utility of LLMs in single tasks~\cite{yang2023large,zhang2023chatgpt} (e.g., recommendation) or single categories of tasks~\cite{li2023ecomgpt} (e.g., e-commerce authoring).
%
However, adapting LLMs as universal \mbox{e-commerce} models for diverse tasks remains largely under-explored.
%
Recent work~\cite{li2023ecomgpt} aims to develop \mbox{e-commerce} LLMs.
%
Though promising, as will be shown in our experiments (Section~\ref{sec:exp_results:in_domain}), 
the performance of existing \mbox{e-commerce} LLMs lags far behind task-specific expert models on widely performed tasks, and thus, could suffer from limited utilities in real-world applications.
%The potential of LLMs in universal \mbox{e-commerce} modeling still remains largely under-explored.
%
%Recent study~\cite{li2023ecomgpt} shows the versatility of LLMs in diverse \mbox{e-commerce} tasks. 
%
%However, it focuses on studying the generalizability of LLMs to new, unseen tasks.
%
%The effectiveness of LLMs, especially when compared to the expert models, in realistic, widely performed \mbox{e-commerce} tasks is still not clear.
%

%In this paper, we study the effectiveness of LLMs as universal \mbox{e-commerce} models 
%
%In this paper, we develop a series of \mbox{e-commerce} LLMs, denoted as \method, using instruction tuning~\cite{zhang2023instruction}.
%
In this paper, we develop a series of effective LLMs specifically for \mbox{e-commerce}, denoted as \method, using instruction tuning~\cite{zhang2023instruction}.
%
Particularly, we construct an instruction dataset for \mbox{e-commerce}, denoted as \dataset.
%
\dataset broadly covers 10 diverse tasks of 4 task categories to enable versatile LLMs for \mbox{e-commerce}.
%
Different from the instruction data introduced in existing work~\cite{li2023ecomgpt,shi2023llama}, 
\dataset considers only real data and undergoes rigorous scrutiny for high quality.
%
In addition, to the best of our knowledge, \dataset is the only \mbox{open-source} \mbox{e-commerce} instruction dataset that could significantly advance the research on LLMs for \mbox{e-commerce}. 
%
Table~\ref{tbl:paper_comparison} presents a detailed comparison between \dataset and the \mbox{e-commerce} instruction dataset in existing work~\cite{shi2023llama,li2023ecomgpt}.
%
With broad coverage and high quality, as will be shown in our experiments, 
\dataset could enable versatile and effective e-commerce LLMs.
%

==> tables/user_OOD_SA_SR.tex <==
\begin{table*}[!h]
  \caption{Overall Performance in User OOD Evaluation}
  \centering
  \label{tbl:overall_user_ood}
  \footnotesize
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{0pt}}l@{\hspace{15pt}}
        %
	  @{\hspace{15pt}}c@{\hspace{15pt}}
        @{\hspace{15pt}}c@{\hspace{0pt}}
      }
      \toprule
      \multirow{2}{*}{Model} & \SA &\SR \\
      \cmidrule(lr){2-3}
      & Macro F1 & HR@1 \\
      \midrule
      GPT-4 Turbo & 0.510 & 0.198 \\
      Gemini Pro & 0.455 & 0.116 \\
      Claude 2.1 & 0.370 & 0.036 \\
      Llama-2 13B-chat & 0.178 & 0.050 \\
      Mistral-7B Instruct-v0.2 & 0.439 & 0.108 \\
      EcomGPT & 0.178 & 0.023 \\
      Expert Model & 0.567 & 0.081 \\
      \midrule
      \methodL & 0.628 & 0.273 \\
      \methodB & 0.640 & 0.280 \\
      \methodS & 0.566 & 0.241 \\         
      \bottomrule
      \end{tabular}
      \begin{tablenotes}[normal,flushleft]
      \begin{footnotesize}
      \item
     	\xn{annotations... this table should go to Appendix}
      \par
      \end{footnotesize}
      %\end{scriptsize}
      \end{tablenotes}
%  \vspace{-10pt}
  \end{threeparttable}
\end{table*}

